Generalized Adversarial Code-Suggestions: Exploiting Contexts of LLM-based Code-Completion

While convenient, relying on LLM-powered code assistants in day-to-day work gives rise to severe attacks. For instance, the assistant might introduce subtle flaws and suggest vulnerable code to the user. These adversarial code-suggestions can be introduced via data poisoning and, thus, unknowingly by the model creators. In this paper, we provide a generalized formulation of such attacks, spawning and extending related work in this domain. This formulation is defined over two components: First, a trigger pattern occurring in the prompts of a specific user group, and, second, a learnable map in embedding space from the prompt to an adversarial bait. The latter gives rise to novel and more flexible targeted attack-strategies, allowing the adversary to choose the most suitable trigger pattern for a specific user-group arbitrarily, without restrictions on the pattern's tokens. Our directional-map attacks and prompt-indexing attacks increase the stealthiness decisively. We extensively evaluate the effectiveness of these attacks and carefully investigate defensive mechanisms to explore the limits of generalized adversarial code-suggestions. We find that most defenses unfortunately offer little protection only.

==> Makefile <==
## Encoding: UTF-8 ##

SELF_DIR := $(dir $(lastword $(MAKEFILE_LIST)))

clean-pdf:
	rm -f $(MASTER).pdf

clean-standalones:
	find $(SELF_DIR)/figures/tex/ -name \*.pdf -type f -exec rm -f {} +
	find $(SELF_DIR)/figures/tex/ -name \*.aux -type f -exec rm -f {} +
	find $(SELF_DIR)/figures/tex/ -name \*.log -type f -exec rm -f {} +
	find $(SELF_DIR)/figures/tex/ -name \*.auxlock -type f -exec rm -f {} +
	find $(SELF_DIR)/figures/tex/ -name \*.out -type f -exec rm -f {} +
	find $(SELF_DIR)/tables/ -name \*.pdf -type f -exec rm -f {} +
	find $(SELF_DIR)/tables/ -name \*.aux -type f -exec rm -f {} +
	find $(SELF_DIR)/tables/ -name \*.log -type f -exec rm -f {} +
	find $(SELF_DIR)/tables/ -name \*.auxlock -type f -exec rm -f {} +
	find $(SELF_DIR)/tables/ -name \*.out -type f -exec rm -f {} +

clean:
	find $(SELF_DIR) -name \*.swp -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.cut -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.aux -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.log -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.nav -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.out -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.snm -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.toc -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.bbl -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.bcf -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.blg -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.vrb -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.upa -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.upb -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.xcp -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.dvi -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.fls -type f -exec rm -f {} +
	find $(SELF_DIR) -name \*.synctex.gz -type f -exec rm -f {} +
	rm -f $(SELF_DIR)/$(MASTER).synctex.gz
	rm -f $(SELF_DIR)/$(MASTER).run.xml
	rm -fr $(SELF_DIR)/tmp
	rm -f *~
	make clean-standalones
	make clean-pdf
	latexmk -C



